MobileNetV4 -- Universal Models for the Mobile Ecosystem

We present the latest generation of MobileNets, known as MobileNetV4 (MNv4), featuring universally efficient architecture designs for mobile devices. At its core, we introduce the Universal Inverted Bottleneck (UIB) search block, a unified and flexible structure that merges Inverted Bottleneck (IB), ConvNext, Feed Forward Network (FFN), and a novel Extra Depthwise (ExtraDW) variant. Alongside UIB, we present Mobile MQA, an attention block tailored for mobile accelerators, delivering a significant 39% speedup. An optimized neural architecture search (NAS) recipe is also introduced which improves MNv4 search effectiveness. The integration of UIB, Mobile MQA and the refined NAS recipe results in a new suite of MNv4 models that are mostly Pareto optimal across mobile CPUs, DSPs, GPUs, as well as specialized accelerators like Apple Neural Engine and Google Pixel EdgeTPU - a characteristic not found in any other models tested. Finally, to further boost accuracy, we introduce a novel distillation technique. Enhanced by this technique, our MNv4-Hybrid-Large model delivers 87% ImageNet-1K accuracy, with a Pixel 8 EdgeTPU runtime of just 3.8ms.

==> res/imagenet-classification-table.tex <==
% % Generated by: https://colab.corp.google.com/drive/1Y0KSVh-9Ukcssj76lr8sUiZfBJxB5zO_?usp=sharing
% \begin{table}
% \caption{ImageNet Classification Results}
% \label{in_cls}
% \begin{tabular}{llllllll}
% \toprule
%  & Phone Model & \multicolumn{3}{c}{Pixel 6} & \multicolumn{3}{c}{Pixel 8} \\
%  & Executor & CPU & GPU & EdgeTPU & CPU & GPU & EdgeTPU \\
%  & Precision & int8 & float & int8 & int8 & float & int8 \\
% \midrule
% Model Family & Top-1 &  \multicolumn{6}{c}{Median Model Latency (ms)} \\
% \midrule
% \multirow[c]{2}{*}{EfficientFormer} & 77.80 & 21.70 & - & - & 20.83 & - & - \\
%  & 81.00 & 55.55 & - & - & 54.27 & - & - \\
% \multirow[c]{2}{*}{EfficientFormer++} & 79.40 & 20.76 & - & - & 19.60 & - & - \\
%  & 82.40 & 56.52 & - & - & 60.22 & - & - \\
% MNv4 - Small & 73.75 & 2.84 & 5.26 & 0.71 & 2.86 & 8.47 & 0.94 \\
% MNv4 - Medium & 79.71 & 13.96 & 11.64 & 1.51 & 13.94 & 18.45 & 1.58 \\
% MNv4 - Large & 82.61 & 72.93 & 30.99 & 4.31 & 77.35 & 33.12 & 3.84 \\
% MobileNetMultiAVG & 76.23 & 6.90 & 8.59 & 1.00 & 7.28 & 11.21 & 1.11 \\
% \multirow[c]{2}{*}{MobileNetMultiMAX} & 77.94 & 10.64 & 11.62 & 1.33 & 11.24 & 15.82 & 1.31 \\
%  & 78.48 & 16.86 & 16.53 & 1.94 & 17.39 & 17.90 & 1.50 \\
% MobileNetV1 & 74.00 & 7.31 & 6.35 & 0.91 & 8.19 & 10.78 & 1.13 \\
% MobileNetV3Large & 75.64 & 5.43 & 7.37 & 1.34 & 5.87 & 10.15 & 1.25 \\
% MobileNetV3Small & 68.07 & 1.94 & 4.44 & 0.88 & 2.03 & 8.21 & 1.05 \\
% \multirow[c]{5}{*}{MobileOne} & 71.40 & 4.92 & 4.42 & 0.74 & 5.67 & 7.63 & 0.91 \\
%  & 75.90 & 10.66 & 8.72 & 0.98 & 11.26 & 12.42 & 1.29 \\
%  & 77.40 & 15.55 & 11.10 & 1.28 & 15.42 & 12.78 & 1.52 \\
%  & 78.10 & 21.31 & 17.10 & 1.45 & 22.28 & 20.87 & 1.80 \\
%  & 79.40 & 32.75 & 19.47 & 2.31 & 34.09 & 23.03 & 2.58 \\
% \bottomrule
% \end{tabular}
% \end{table}

% % Generated by: https://colab.corp.google.com/drive/1Y0KSVh-9Ukcssj76lr8sUiZfBJxB5zO_?usp=sharing
% \begin{table}
% \caption{ImageNet Classification Results with Gmean}
% \label{in_cls_gmean}
% \begin{tabular}{llc}
% \toprule
%  &  & Normalized Latency \\
% Model Family & Top-1 &  \\
% \midrule
% MobileNetV3Small & 68.07 & 0.48 \\
% MNv4 - Small & 73.75 & 0.57 \\
% MobileOne & 71.40 & 0.71 \\
% MobileNetV3Large & 75.64 & 0.86 \\
% MobileNetMultiAVG & 76.23 & 0.94 \\
% MobileNetV1 & 74.00 & 1.00 \\
% MobileOne & 75.90 & 1.26 \\
% MobileNetMultiMAX & 77.94 & 1.31 \\
% MNv4 - Medium & 79.71 & 1.59 \\
% MobileOne & 77.40 & 1.63 \\
% MobileNetMultiMAX & 78.48 & 1.84 \\
% \multirow[c]{2}{*}{MobileOne} & 78.10 & 2.20 \\
%  & 79.40 & 3.14 \\
% MNv4 - Large & 82.61 & 5.02 \\
% EfficientFormer++ & 79.40 & 6.85 \\
% \multirow[c]{2}{*}{EfficientFormer} & 77.80 & 7.22 \\
%  & 81.00 & 19.79 \\
% EfficientFormer++ & 82.40 & 20.81 \\
% \bottomrule
% \end{tabular}
% \end{table}

% Generated by: https://colab.corp.google.com/drive/1Y0KSVh-9Ukcssj76lr8sUiZfBJxB5zO_?usp=sharing
%but edited substantially in this doc so don't replace
% Table from CVPR submission
% \begin{table}[!ht]
% \footnotesize
% \setlength\tabcolsep{1.5pt}
% \begin{tabular}{l c c c c c c c}
% \toprule
%  & & & & & \multicolumn{2}{c}{\scriptsize{Latency (ms)}} \\
%  & & \scriptsize{Top-1} &  \scriptsize{Params} & \scriptsize{Macs} & \scriptsize{Pixel 6} & \scriptsize{Pixel 8} \\
% %  &  &  &  & Executor & CPU & EdgeTPU \\
% %  &  &  &  & Precision & int8 & int8 \\
% \scriptsize{Model} & \scriptsize{Top-1} &  \scriptsize{Open} & \scriptsize{(M)} & \scriptsize{(G)} &  \scriptsize{CPU} & \scriptsize{EdgeTPU} \\
% \midrule
% MNv3-0.5xL~\cite{mobilenet_v3} & 69.2 & - & 2.7 & 0.1 & 2.4 & 0.8 \\
% MobileOne-S0~\cite{vasu2023mobileone}  & 71.4 & 72.5 & 2.1 & 0.3 & 4.2 & 0.7 \\
% \textbf{MNv4-Conv-S} & \textbf{73.8} & \textbf{75.5$^{\star}$} & \textbf{3.8} & \textbf{0.2} & \textbf{2.4} & \textbf{0.7} \\
% MobileNet-v1~\cite{howard2017mobilenets} & 74.0 & - & 4.2 & 0.6 & 6.1 & 0.9 \\
% \midrule
% FastViT-T8$^{\dag}$~\cite{vasu2023fastvit} & 75.6 & 76.7 & 3.6 & 0.7 & 49.3 & 1.3 \\
% MobileOne-S4~\cite{vasu2023mobileone} & 79.4 & 81.4 & 14.8 & 1.5 & 26.7 & 1.7 \\
% FastViT-S12$^{\dag}$~\cite{vasu2023fastvit} & 79.8 & 80.9 & 8.8 & 1.8 & 86.5 & 1.8 \\
% E-FormerV2-S2$^{\dag}$~\cite{efficientformerv2} & - & 82.0 & 12.6 & 1.3 & 57.2 & - \\
% \textbf{MNv4-Conv-M} & \textbf{79.9} & \textbf{82.7$^{\star}$} & \textbf{9.2} & \textbf{1.0} & \textbf{11.4} & \textbf{1.1} \\
% \midrule
% FastViT-SA12$^{\dag}$~\cite{vasu2023fastvit}  & 80.6 & 81.0 & 10.9 & 1.9 & 86.5 & 2.0 \\
% \textbf{MNv4-Hybrid-M} & \textbf{80.7} & \textbf{83.7$^{\star}$} & \textbf{10.5} & \textbf{1.2} & \textbf{14.3} & \textbf{1.5}\\
% \midrule
% E-FormerV2-L$^{\dag}$~\cite{efficientformerv2} & - & 83.5 & 26.1 & 2.6 & 117.7 & - \\
% FastViT-SA24$^{\dag}$~\cite{vasu2023fastvit} & 82.6 & 83.4 & 20.6 & 3.8 & 171.6 & 3.2 \\
% \textbf{MNv4-Conv-L} & \textbf{82.9} & \textbf{85.9$^{\star}$} & \textbf{31} & \textbf{5.9} & \textbf{59.9} & \textbf{2.4} \\
% ConvNext-S$^{\dag}$~\cite{convnext} & 83.1 & 84.6$^{\star}$ & 50 & 8.7 & 314.9 & 3.7 \\
% \midrule
% NextViT-B $^{\dag}$~\cite{li2022nextvit} & 83.2 & 85.1 & 44.8 & 8.3 & - & - \\
% \textbf{MNv4-Hybrid-L$^{\dag}$} & \textbf{83.4} & \textbf{86.6$^{\star}$/87.0$^{\diamond}$} & \textbf{35.9} & \textbf{7.2} & \textbf{87.6} & \textbf{3.8} \\
% FastViT-SA36$^{\dag}$~\cite{vasu2023fastvit} & 83.6 & 84.2 & 30.4 & 5.6 & 241.6 & 4.3 \\
% \bottomrule
% \end{tabular}
% \caption{ImageNet-1K~\cite{imagenet} classification results. Median latency is reported. $\dag$=GeLu, $\ddag$=HardSwish, otherwise ReLU is used. $^{\star}$ indicates additional data was used.
% $^{\diamond}$ indicates additional pretraining with JFT~\cite{sun2017revisiting}.
% }
% \label{tab:classification_results}
% \end{table}



% EDIT from mdelakis: comment this out and replace with table below
% \begin{table}[tbp]
% \small
% % \setlength\tabcolsep{1.5pt}
% \scriptsize
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l c c c c c c c c c c}
% \toprule
%   & & & & \multicolumn{6}{c}{Latency (ms)} \\
%  & &  Params & MACs & Pixel 6 & Pixel 8  & iPhone 13 & Pixel 4 & Pixel 7 & Samsung S23 \\
% Model & Top-1 & (M) & (G) &  CPU & EdgeTPU & CoreML & Hexagon
% & GPU & GPU \\
% \midrule
% MobileNet-V2-0.5x~\cite{mobilenet_v2} & 66  & 2.0 & 0.1 & 2.4 & 0.7 & - & 2.9 & 9.9 & 2.6 \\
% MobileNet-V3-0.5xL~\cite{mobilenet_v3} & 69.2 & 2.7 & 0.1 & 2.4 & 0.8 & - & 3.4 & 10.3 & 3.0 \\
% MobileOne-S0~\cite{vasu2023mobileone}  & 71.4  & 2.1 & 0.3 & 4.2 & 0.7 & 0.5 & 2.8 & 16.3 & 2.3 \\
% MobileNet-V2~\cite{mobilenet_v2} & 73.4  & 3.5 & 0.3 & 5.0 & 0.8 & - & 3.9 & 15.0 & 3.5 \\
% \textbf{MNv4-Conv-S} & \textbf{73.8} & \textbf{3.8} & \textbf{0.2} & \textbf{2.4} & \textbf{0.7} & \textbf{0.5} & \textbf{2.9} & \textbf{11.8} & \textbf{2.7} \\
% MobileNet-V1~\cite{howard2017mobilenets} & 74.0 & 4.2 & 0.6 & 6.1 & 0.9 & - & 3.2 & 14.0 & 2.9 \\
% \midrule
% FastViT-T8$^{\dag}$~\cite{vasu2023fastvit} & 75.6 & 3.6 & 0.7 & 49.3 & 1.3 & 0.7 & \textit{Failed} & 38.4 & 25.5 \\
% MultiHardware-1.5x~\cite{mobilenet_multi} & 78.2 & 10.0 & 1.0 & 12.0 & 1.1 & - & 6.1 & 20.3 & 4.5 \\
% MobileNet-V2-2.0x~\cite{mobilenet_v2} & 78.4 & 11.2 & 1.1 & 13.9 & 1.1 & - & 6.8 & 20.9 & 5.14 \\
% MobileOne-S4~\cite{vasu2023mobileone} & 79.4 & 14.8 & 1.5 & 26.7 & 1.7 & 1.5 & 9.0 & 24.4 & 7.0 \\
% FastViT-S12$^{\dag}$~\cite{vasu2023fastvit} & 79.8 & 8.8 & 1.8 & 86.5 & 1.8 & 1.3 & \textit{Failed} & 73.8 & 45.5 \\
% % EfficientFormerV2-S2$^{\dag}$~\cite{efficientformerv2} & - & 12.6 & 1.3 & 57.2 & -  & - & - & - & -\\
% \textbf{MNv4-Conv-M} & \textbf{79.9} & \textbf{9.2} & \textbf{1.0} & \textbf{11.4} & \textbf{1.1} & \textbf{1.1} & \textbf{7.2} & \textbf{23.0}  & \textbf{5.1} \\
% \midrule
% FastViT-SA12$^{\dag}$~\cite{vasu2023fastvit}  & 80.6 & 10.9 & 1.9 & 86.5 & 2.0 & 1.6 & \textit{Failed} & 79.8 & 50.9 \\
% \textbf{MNv4-Hybrid-M} & \textbf{80.7}  & \textbf{10.5} & \textbf{1.2} & \textbf{14.3} & \textbf{1.5} & - & \textbf{\textit{Failed}} & \textbf{21.9} & \textbf{7.6} \\
% \midrule
% % E-FormerV2-L$^{\dag}$~\cite{efficientformerv2} & - & 26.1 & 2.6 & 117.7 & - & - & - & - & - \\
% FastViT-SA24$^{\dag}$~\cite{vasu2023fastvit} & 82.6 & 20.6 & 3.8 & 171.6 & 3.2 & 2.6 & \textit{Failed} & 128.9 & 103.2 \\
% \textbf{MNv4-Conv-L} & \textbf{82.9} & \textbf{31} & \textbf{5.9} & \textbf{59.9} & \textbf{2.4} & \textbf{3.0} & \textbf{20.5} & \textbf{38.5} & \textbf{13.3} \\
% \midrule
% ConvNext-S$^{\dag}$~\cite{convnext} & 83.1  & 50 & 8.7 & 314.9 & 3.7 & - & \textit{Failed} & 48.3 & 19.0 \\
% NextViT-B $^{\dag}$~\cite{li2022nextvit} & 83.2 & 44.8 & 8.3 & - & - & - & - & - & - \\
% \textbf{MNv4-Hybrid-L$^{\dag}$} & \textbf{83.4} & \textbf{35.9} & \textbf{7.2} & \textbf{87.6} & \textbf{3.8} & - & \textbf{\textit{Failed}} & \textbf{65.4} & \textbf{18.6} \\
% FastViT-SA36$^{\dag}$~\cite{vasu2023fastvit} & 83.6 & 30.4 & 5.6 & 241.6 & 4.3 & - & \textit{Failed} & 173.1 & 144.6 \\
% \bottomrule
% \end{tabular}
% }%end resizebox
% \caption{
% Classification results of models training on ImageNet-1K~\cite{imagenet} exclusively, along with benchmarking results on an expanded list of devices.
% % Median latency is reported. 
% ``$-$'' indicates that we did not benchmark a model due to missing corresponding model file for a platform. ``\textit{Failed}'' indicates that we have tried to benchmark the model on a device but failed. 
% % $\dag$=GeLu, $\ddag$=HardSwish, otherwise ReLU is used. $^{\star}$ indicates additional data was used.
% % $^{\diamond}$ indicates additional pretraining with JFT~\cite{sun2017revisiting}.
% }
% \label{tab:classification_results}
% \end{table}
 

% Results from https://docs.google.com/spreadsheets/d/1i-i-otraVxpQ8uHPkJ2LylG6JBNHTlILvOku2K3giK8/edit?resourcekey=0-tu_8eC6n3apCJYYkDhe5aQ#gid=336652603
% and https://docs.google.com/spreadsheets/d/1i-i-otraVxpQ8uHPkJ2LylG6JBNHTlILvOku2K3giK8/edit?resourcekey=0-tu_8eC6n3apCJYYkDhe5aQ#gid=2016040296


 
%  FV-MA36 $\times$ & 83.9 & 84.6 & 42.7&7.9 & - &- \\
% EV-B3-r224 $\diamond$  & 83.5 & - & 49.0&4.0 & - &- \\
%  \textbf{MNV4-H-L $\diamond$ } & - & 86.4 & 35.9&7.2 & - & 3.2 \\
%  NV-L $\times$ & 83.6 & 85.4 & 57.8&10.8 & - &- \\
% MobileNet-MultiAverage-1.0 & 76.23 & - & 4.93 & 432.45 & 6.05 & 0.96 \\
% MobileNet-MultiMax-1.5 & 77.94 & - & 8.88 & 764.03 & 8.89 & 1.12 \\
% MobileNet-MultiMax-2.0 & 78.48 & - & 14.86 & 1339.05 & 14.07 & 1.28 \\
% MobileNetV3-Small & 68.07 & - & 2.54 & 56.51 & 1.79 & 0.93 \\
% MobileNet-EdgeTPUV2-L & 79.00 & - & 10.89 & 2530.79 & 25.08 & 1.61 \\
% MobileNet-EdgeTPUV2-M & 78.43 & - & 8.43 & 1835.64 & 16.87 & 1.45 \\
% MobileNet-EdgeTPUV2-S & 77.36 & - & 5.96 & 1198.00 & 11.83 & 1.24 \\
% MobileNet-EdgeTPUV2-T & 74.66 & - & 3.74 & 512.45 & 5.88 & 1.02 \\
% MobileNet-EdgeTPUV2-XS & 75.79 & - & 4.44 & 707.48 & 7.27 & 1.09 \\
% MobileOne-S1 & 75.90 & - & 4.76 & 825.06 & 8.74 & 1.10 \\
% MobileOne-S2 & 77.40 & - & 7.81 & 1298.43 & 13.21 & 1.27 \\
% MobileOne-S3 & 78.10 & - & 10.08 & 1895.79 & 17.40 & 1.49 \\
% MobileOne-S4 & 79.40 & - & 14.84 & 2979.27 & 27.29 & 2.09 \\


% Old version without shortened names
% % Generated by: https://colab.corp.google.com/drive/1Y0KSVh-9Ukcssj76lr8sUiZfBJxB5zO_?usp=sharing
% %but edited substantially in this doc so don't replace
% \begin{table}[ht]
% \small
% \caption{ImageNet Classification Results}
% \label{in_cls}
% \begin{tabular}{lccccc}
% \toprule
%  &  &  & \multicolumn{2}{r}{Median Latency (ms)} \\
%  & Top-1 / &  Mparams / & Pixel 7 & Pixel 8 \\
% %  &  &  &  & Executor & CPU & EdgeTPU \\
% %  &  &  &  & Precision & int8 & int8 \\
% Name (Activation) & Extra Data & Gmacs & CPU & EdgeTPU \\
% \midrule
% MobileNetV1-1.0 (ReLU) & 74.0 / \hspace{.2cm}-\hspace{.2cm} & 4.2 / 0.6 & 6.04 & 0.92 \\
% MobileNetV3-Large (Hard-Swish) & 75.6 / \hspace{.2cm}-\hspace{.2cm} & 5.5 / 0.2 & 4.73 & 1.09 \\
% MobileOne-S0 (ReLU) & 71.4 / \hspace{.2cm}-\hspace{.2cm} & 2.1 / 0.3 & 4.16 & 0.81 \\
% \textbf{MobileNetV4-Small (ReLU)} & 73.8 / 74.9 & 3.8 / 0.2 & 2.40 & 0.84 \\
% FastViT-T8 (GeLU) & 75.6 / 76.7 & 3.6 / 0.7 & - & - \\
% FastViT-S12 (GeLU) & 79.8 / 80.9 & 8.8 / 1.8 & - & - \\
% EfficientFormerV2-S2 (GeLU) & \hspace{.2cm}-\hspace{.2cm} / 82.0 & 12.6 / 1.0 & - & - \\
% \textbf{MobileNetV4-Medium (ReLU)} & 79.7 / \hspace{.2cm}-\hspace{.2cm} & 9.7 / 1.1 & 12.1 & 1.1 \\
% \midrule
% EfficientFormerV2-L (GeLU) & \hspace{.2cm}-\hspace{.2cm} / 83.5 & 26.1 / 2.6 & - & - \\
% ConvNext-S (GeLU) & 83.1 / 84.6 & 50.0 / 8.7 & - & - \\
% Next-ViT-B (GeLU) & 83.2 / 85.1 & 44.8 / 8.3 & - & - \\
% FastViT-SA36 (GeLU) & 83.6 / 84.2 & 30.4 / 5.6 & - & - \\
% \textbf{MobileNetV4-Large (ReLU)} & 82.9 / 85.9 & 30.9 / 5.9 & 60.6 & 2.35 \\
% \midrule
% Next-ViT-L (GeLU) & 83.6 / 85.4 & 57.8 / 10.8 & - & - \\
% FastViT-MA36 (GeLU) & 83.9 / 84.6 & 42.7 / 7.9 & - & - \\
% EfficientVIT-B3-r224 (ReLU) & 83.5 / \hspace{.2cm}-\hspace{.2cm} & 49.0 / 4.0 & - & - \\
% \textbf{MobileNetV4-Hybrid-Large (ReLU)} & \hspace{.2cm}-\hspace{.2cm} / 86.4 & 35.9 / 7.2 & 78.8 & 3.2 \\
% \textbf{MobileNetV4-Hybrid-Large (GeLU)} & 83.4 / 87.0 & 35.9 / 7.2 & 82.0 & 3.75 \\


% % MobileNet-MultiAverage-1.0 & 76.23 & - & 4.93 & 432.45 & 6.05 & 0.96 \\
% % MobileNet-MultiMax-1.5 & 77.94 & - & 8.88 & 764.03 & 8.89 & 1.12 \\
% % MobileNet-MultiMax-2.0 & 78.48 & - & 14.86 & 1339.05 & 14.07 & 1.28 \\
% % MobileNetV3-Small & 68.07 & - & 2.54 & 56.51 & 1.79 & 0.93 \\
% % MobileNet-EdgeTPUV2-L & 79.00 & - & 10.89 & 2530.79 & 25.08 & 1.61 \\
% % MobileNet-EdgeTPUV2-M & 78.43 & - & 8.43 & 1835.64 & 16.87 & 1.45 \\
% % MobileNet-EdgeTPUV2-S & 77.36 & - & 5.96 & 1198.00 & 11.83 & 1.24 \\
% % MobileNet-EdgeTPUV2-T & 74.66 & - & 3.74 & 512.45 & 5.88 & 1.02 \\
% % MobileNet-EdgeTPUV2-XS & 75.79 & - & 4.44 & 707.48 & 7.27 & 1.09 \\
% % MobileOne-S1 & 75.90 & - & 4.76 & 825.06 & 8.74 & 1.10 \\
% % MobileOne-S2 & 77.40 & - & 7.81 & 1298.43 & 13.21 & 1.27 \\
% % MobileOne-S3 & 78.10 & - & 10.08 & 1895.79 & 17.40 & 1.49 \\
% % MobileOne-S4 & 79.40 & - & 14.84 & 2979.27 & 27.29 & 2.09 \\
% \bottomrule
% \end{tabular}
% \end{table}
